SoK: The Ghost Trilemma

Trolls, bots, and sybils distort online discourse and compromise the security of networked platforms. User identity is central to the vectors of attack and manipulation employed in these contexts. However it has long seemed that, try as it might, the security community has been unable to stem the rising tide of such problems. We posit the Ghost Trilemma, that there are three key properties of identity -- sentience, location, and uniqueness -- that cannot be simultaneously verified in a fully-decentralized setting. Many fully-decentralized systems -- whether for communication or social coordination -- grapple with this trilemma in some way, perhaps unknowingly. In this Systematization of Knowledge (SoK) paper, we examine the design space, use cases, problems with prior approaches, and possible paths forward. We sketch a proof of this trilemma and outline options for practical, incrementally deployable schemes to achieve an acceptable tradeoff of trust in centralized trust anchors, decentralized operation, and an ability to withstand a range of attacks, while protecting user privacy.

==> trilemma.tex <==
\section{Trilemma}
\prs{graphic showing the components of the design space. Components should map to any table that details a particular set of design choices.}
%\paragraph{Using latency to figure out the location}
%The main components that any attestation procedure should have include some way to check

\subsection{System properties and Ideal world functionality}
\begin{itemize}
    \item The person is physically present at a specific location and at a specific moment in time (\textbf{sentience of the user}).
    \item The identity of this person leads back to a credible profile of existence, i.e., we want to know that the entity claiming the account is indeed a person at the expected location at the time (\textbf{location of the user}).
    %\textcolor{blue}{to distinguish it clearly from liveness, this should stated as a function of liveness}
    \item A way to bind the accounts being attested to the individual showing up claiming to own said accounts to enable limiting of the number of verified accounts per individual. We want to establish the \textbf{uniqueness of the user} without necessarily deciphering the actual identity of the individual. One person cannot be allowed to verify unlimited number of accounts. If that could happen, the adversary's bottleneck of limited physical presence on the US soil would not remain a bottleneck anymore.
    %\textcolor{blue}{Apart from formulating the sybil issue, this requires formulating the privacy property. Real identity is indistinguishable to every other participant including the adversary from a random one with high probability}
\end{itemize}

\paragraph{Ideal world functionality}
We present how a verifier $\mathcal{V}$ can establish user sentience, attribute location and confirm uniqueness assuming the existence of a trusted party $\mathcal{F}$.

\begin{figure*}[!ht]
\scalebox{0.75}{
\begin{tikzpicture}
\definecolor{black}{rgb}{0 0 0}
\tikzstyle{rec} = [rectangle,rounded corners,thick,draw=black,fill=white] 
\node[rec,text=black,inner sep=3mm,drop shadow] (th)
	{\parbox{1.3\textwidth}{
\underline{Attributing location}
$\mathcal{V}$ computes user location based on two intuitions: that websites often provide geographical location of associated entities and relative network delays correspond with geographical distances~\cite{wang2011towards}. A website of a particular location might be hosted in another site but an institutional email server, for example, is more likely to be on the same location and can be used as a landmark. A list of such landmarks all over the country/world were obtained by the authors. The three steps in their method to associate a landmark to a target:
\begin{itemize}
    \item Find the coarse grained region for the targeted IP by measuring delays to pings from ping servers at several vantage points. The measured delays give the geographical distances and they create a rough intersecting region from the collected data following the CBG approach \cite{gueye2006constraint}.
    \item Use passive landmarks to get a finer grained IP: Populate the intersection with the landmarks. Then they estimate the distance b/w the landmark(s) and the IP indirectly through available vantage point servers and routers in the locality. Typically the estimated distance is still inflated (often by three orders in magnitude according to this study). This creates a new smaller intersection. 
    \item Select the landmark with the minimum delay to the target and associate its location to the target.
\end{itemize}
The verification of whether the landmark is actually at the given location is done through ZIP code verification and CDN network listings. 
%and they claim it removes a majority of the possible errors.
The location can be obtained for a host by a server implementing this protocol. \\
%However, we will also need to bind this with a liveness verifier which would simultaneously check the liveness of the user at the time during which its location is known.
\underline{Attributing sentience} $\mathcal{V}$ Checks if the user is a sentient being who can pass the Turing test, i.e., express their capability to understand and propagate multi dimensional ideologies and actions at \mathcal{F}.\\
\underline{Attributing uniqueness} $\mathcal{V}$ maps user identity with unique governmental identifier. For a $k$-shot user operation, the identifier is checked $k$ times for preventing Sybils. 

}};


\node[rec,text=black!95,anchor=south west,xshift=3mm,yshift=-1mm] 
	at (th.north west) {\small \textbf{Ideal World Functionality $\mathcal{F}$}};

\end{tikzpicture}}
\vspace{-6mm}
\caption{The ideal world functionality for a verifier $\mathcal{V}$ using a centralized trusted party $\mathcal{F}$ to attribute sentience, location and uniqueness }
\label{algo:ideal-world}
\vspace{-2mm}
\end{figure*}
%

\paragraph{On the hardness of attributing sentience, location and uniqueness}
We show that the ideal world functionality $\mathcal{F}$ (Figure~\ref{algo:ideal-world}) described cannot be achieved without a trusted functionality: specifically, it is impossible for an external verifier to deterministically attribute sentience, attest user location and perform privacy-preserving identity verification in a decentralized system.
\begin{lemma}
Consider a verifier $\mathcal{V}$ and an asynchronous decentralized system with permissionless participation for its participants. Then it is impossible for $\mathcal{V}$ to attribute sentience, user location and uniqueness in a finite amount of time with respect to $\mathcal{F}$. 
\end{lemma}
%
\begin{proof}
Suppose by contradiction that there exists a verifier $\mathcal{V}$ that can attribute sentience, user location and perform identity verification in a finite amount of time as specified by $\mathcal{F}$.
The proof argument is derived by showing that in order for $\mathcal{V}$ to attribute sentience, user location and perform identity verification in a decentralized system, \emph{consensus} will have to be achieved by all the participants in the system. Moreover, consensus will have to achieved in a finite amount of time independent of the relative speeds of the participants in the verification protocol: so-called \emph{wait-free} consensus~\cite{FLP85}. 


\end{proof}



